Deep Imbalanced Time-series Forecasting via Local Discrepancy Density

Time-series forecasting models often encounter abrupt changes in a given period of time which generally occur due to unexpected or unknown events. Despite their scarce occurrences in the training set, abrupt changes incur loss that significantly contributes to the total loss. Therefore, they act as noisy training samples and prevent the model from learning generalizable patterns, namely the normal states. Based on our findings, we propose a reweighting framework that down-weights the losses incurred by abrupt changes and up-weights those by normal states. For the reweighting framework, we first define a measurement termed Local Discrepancy (LD) which measures the degree of abruptness of a change in a given period of time. Since a training set is mostly composed of normal states, we then consider how frequently the temporal changes appear in the training set based on LD. Our reweighting framework is applicable to existing time-series forecasting models regardless of the architectures. Through extensive experiments on 12 time-series forecasting models over eight datasets with various in-output sequence lengths, we demonstrate that applying our reweighting framework reduces MSE by 10.1% on average and by up to 18.6% in the state-of-the-art model.

==> Figures/suple-rect-series-broken.tex <==
\begin{figure}[h!]
\begin{center}
  \includegraphics[width=\linewidth]{Figures/images/r-figure3-rect-broken-period.png}
\end{center}
\vspace{-5mm}
\caption{\js{Forecasting results of Autoformer on three datasets: ETTm1, ETTm2, and Weather. The first row shows the forecasting results of the baseline without our ReLD and the second row shows those with our ReLD.}}
\label{fig:suple-rect-broken}
\end{figure}

==> Tables/ablation_ld.tex <==
\begin{table}[]
\caption{
% Ablation of assigning weight to mitigate imbalanced loss by abrupt changes. 
Ablation study on our reweighting framework using ETTm2.
% We compare our re-weighting frameworks: the inverse ofiLD-based andiLD density-based. 
We compare models 1) without our framework, 2) reweighting inversely to LD, and 3) reweighting based on LD density.
% ReLD shows more consistent and superior results than the inverse ofiLD on ETTm2 dataset in multivariate setting.
ReLD shows more consistent and superior results compared to reweighting inversely to LD in the multivariate setting.
}

\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc||cc}
\toprule
Models     & \multicolumn{3}{c}{Pyraformer}             & \multicolumn{3}{c}{SCINet}             & \multicolumn{3}{c}{Autoformer}                 & \multicolumn{3}{c||}{Informer} & \multicolumn{2}{c}{Averaged Imp.} \\  

\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-15}


Predict-O & base &iLD & \multicolumn{1}{l|}{ReLD} & base &iLD & \multicolumn{1}{l|}{ReLD} & base &iLD & \multicolumn{1}{l|}{ReLD} & base    &iLD    & ReLD   &iLD     & ReLD      \\ \midrule

48        &  \makecell{ 0.2806 \\\scriptsize$\pm$0.0215 } & \makecell{ 0.2793 \\\scriptsize$\pm$0.0233 } & \makecell{\textbf{0.2200} \\\scriptsize$\pm$0.0283 } & \makecell{ 0.2826 \\\scriptsize$\pm$0.0695 } & \makecell{ 0.2692 \\\scriptsize$\pm$0.0341 } & \makecell{ \textbf{0.2245} \\\scriptsize$\pm$0.0506 } & \makecell{ 0.1708 \\\scriptsize$\pm$0.0051 } & \makecell{ 0.1700 \\\scriptsize$\pm$0.0012 } & \makecell{ \textbf{0.1689} \\\scriptsize$\pm$0.0023 } & \makecell{ 0.2953 \\\scriptsize$\pm$0.0350 } & \makecell{ 0.3021 \\\scriptsize$\pm$0.0437 } & \makecell{ \textbf{0.2143} \\\scriptsize$\pm$0.0188 } & -0.84\% & \textbf{-17.67\%} \\

96        &   \makecell{ 0.3709 \\\scriptsize$\pm$0.1396 } & \makecell{ 0.3416 \\\scriptsize$\pm$0.0596 } & \makecell{ \textbf{0.2480} \\\scriptsize$\pm$0.0164 } & \makecell{ 0.3919 \\\scriptsize$\pm$0.1291 } & \makecell{ 0.3663 \\\scriptsize$\pm$0.1185 } & \makecell{ \textbf{0.2568} \\\scriptsize$\pm$0.0313 } & \makecell{ 0.2934 \\\scriptsize$\pm$0.0691 } & \makecell{ 0.2387 \\\scriptsize$\pm$0.0273 } & \makecell{ \textbf{0.2213} \\\scriptsize$\pm$0.0126 } & \makecell{ 0.4451 \\\scriptsize$\pm$0.0519 } & \makecell{ 0.4515 \\\scriptsize$\pm$0.0479 } & \makecell{\textbf{0.2860} \\\scriptsize$\pm$0.0221 }  & -7.91\% & \textbf{-31.98\%} \\
168       &    \makecell{ 0.5655 \\\scriptsize$\pm$0.0840 } & \makecell{ 0.5648 \\\scriptsize$\pm$0.1060 } & \makecell{ \textbf{0.5515} \\\scriptsize$\pm$0.0586 } & \makecell{ 0.7432 \\\scriptsize$\pm$0.3397 } & \makecell{ 0.6957 \\\scriptsize$\pm$0.4219 } & \makecell{ \textbf{0.4857} \\\scriptsize$\pm$0.1357 } & \makecell{ 0.3095 \\\scriptsize$\pm$0.0130 } & \makecell{ 0.3103 \\\scriptsize$\pm$0.0148 } & \makecell{ \textbf{0.2840} \\\scriptsize$\pm$0.0116 } & \makecell{ 2.2831 \\\scriptsize$\pm$0.1434 } & \makecell{ 2.2613 \\\scriptsize$\pm$0.1218 } & \makecell{ \textbf{1.4531} \\\scriptsize$\pm$0.1662 } & -1.80\% & \textbf{-20.43\%} \\


336       &   \makecell{ 1.6013 \\\scriptsize$\pm$0.3115 } & \makecell{ 1.8544 \\\scriptsize$\pm$0.3478 } & \makecell{ \textbf{1.3296} \\\scriptsize$\pm$0.2605 } & \makecell{ 1.8812 \\\scriptsize$\pm$1.0633 } & \makecell{ 1.9464 \\\scriptsize$\pm$1.0921 } & \makecell{ \textbf{1.5110} \\\scriptsize$\pm$0.5270 } & \makecell{ 0.5084 \\\scriptsize$\pm$0.1483 } & \makecell{ 0.4123 \\\scriptsize$\pm$0.0495 } & \makecell{ \textbf{0.4046} \\\scriptsize$\pm$0.0818 } & \makecell{ 2.4795 \\\scriptsize$\pm$0.1344 } & \makecell{ 2.4891 \\\scriptsize$\pm$0.1496 } & \makecell{ \textbf{1.7639} \\\scriptsize$\pm$0.1074 }  & 0.19\% & \textbf{-21.48\%} \\
720       &  \makecell{ 5.4764 \\\scriptsize$\pm$0.9723 } & \makecell{ 5.7002 \\\scriptsize$\pm$1.2026 } & \makecell{ \textbf{5.0372} \\\scriptsize$\pm$0.6450 } & \makecell{ 4.0937 \\\scriptsize$\pm$2.4575 } & \makecell{ 4.2890 \\\scriptsize$\pm$1.7328 } & \makecell{ \textbf{3.7514} \\\scriptsize$\pm$1.4716 } & \makecell{ 0.5022 \\\scriptsize$\pm$0.0937 } & \makecell{ 0.5200 \\\scriptsize$\pm$0.1333 } & \makecell{ \textbf{0.4257} \\\scriptsize$\pm$0.0527 } & \makecell{ 6.5797 \\\scriptsize$\pm$0.7368 } & \makecell{ 6.3353 \\\scriptsize$\pm$0.8901 } & \makecell{ \textbf{5.7770} \\\scriptsize$\pm$0.6946 }  & 2.17\% & \textbf{-10.95\%} \\  
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\label{tab:ablation-ld}
\end{table}

==> Tables/iclr_uni_main_results.tex <==
\begin{table}[]
\caption{Univariate results with different prediction lengths. The experimental settings are identical to those of multivariate experiments.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccc|cc|cc|cc|cc|cc|cc|cc||c@{}}
\toprule


% \multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{N-BEATS}  & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{LogSparse}  & \multicolumn{2}{c}{Reformer} & \multicolumn{2}{c}{Transformer} & \multicolumn{2}{c}{DeepAR} \\
% \cmidrule{3-18}
% \multicolumn{2}{c}{MSE}                                             & base           & ReLD           & base         & ReLD         & base           & ReLD          & base          & ReLD          & base          & ReLD          & base            & ReLD           & base         & ReLD         & base         & ReLD       \\ \midrule
\multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{FEDformer} & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{Autoformer}  & \multicolumn{2}{c}{N-BEATS} & \multicolumn{2}{c}{Informer}  & \multicolumn{2}{c}{LogSparse} & \multicolumn{2}{c}{Transformer} & \multicolumn{2}{c||}{DeepAR} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Total}}} \\

% \cmidrule{3-18}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
\cmidrule(lr){15-16}
\cmidrule(lr){17-18}

\multicolumn{2}{c}{MSE}                                             & base           & ReLD           & base         & ReLD         & base           & ReLD          & base          & ReLD          & base          & ReLD          & base            & ReLD           & base         & ReLD         & base         & ReLD       \\ \midrule


% ETTm1
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ETTm1}}} & \multicolumn{1}{l|}{96/96}  &0.036 & \textbf{0.035} & 0.082 & 0.058 & 0.058 & 0.052 & 0.085 & 0.066 & 0.105 & 0.083 & 0.105 & 0.058 & 0.089 & 0.060 & 0.179 & 0.085     & \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-15.11\%}}} \\


\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336/168} &0.083 & \textbf{0.066} & 0.129 & 0.122 & 0.088 & 0.072 & 0.077 & 0.070 & 0.181 & 0.158 & 0.192 & 0.161 & 0.221 & 0.196 & 0.200 & 0.199       \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336/336} & 0.081 & \textbf{0.076} & 0.194 & 0.184 & 0.090 & 0.085 & 0.134 & 0.125 & 0.263 & 0.227 & 0.367 & 0.304 & 0.274 & 0.247 & 0.382 & 0.432     \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336/720} &0.109 & \textbf{0.102} & 0.337 & 0.275 & 0.143 & 0.112 & 0.144 & 0.112 & 0.391 & 0.349 & 0.474 & 0.381 & 0.479 & 0.443 & 0.498 & 0.418     \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-8.81\%} & \multicolumn{2}{c|}{-14.61\%} & \multicolumn{2}{c|}{-13.83\%} & \multicolumn{2}{c|}{-15.20\%} & \multicolumn{2}{c|}{-14.58\%} & \multicolumn{2}{c|}{-24.42\%} & \multicolumn{2}{c|}{-15.40\%} & \multicolumn{2}{c|}{-14.05\%} \\ \midrule


% ECL
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ECL}}} & \multicolumn{1}{l|}{96/96}  &0.243 & 0.240 & 0.239 & \textbf{0.234} & 0.440 & 0.424 & 0.303 & 0.295 & 0.269 & 0.272 & 0.281 & 0.282 & 0.301 & 0.283 & 0.917 & 0.786  & \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-3.87\%}}}\\


\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336/168} & 0.304 & 0.299 & 0.255 & \textbf{0.253} & 0.486 & 0.482 & 0.328 & 0.311 & 0.709 & 0.705 & 0.330 & 0.335 & 0.404 & 0.373 & 1.018 & 1.024   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336/336} &0.355 & 0.345 & 0.306 & \textbf{0.296} & 0.463 & 0.439 & 0.425 & 0.386 & 0.801 & 0.743 & 0.399 & 0.316 & 0.443 & 0.424 & 1.202 & 1.280   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336/720} &0.469 & 0.448 & 0.336 & \textbf{0.321} & 0.606 & 0.616 & 0.544 & 0.497 & 0.824 & 0.781 & 0.372 & 0.339 & 0.442 & 0.413 & 1.302 & 1.331   \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       &  \multicolumn{1}{l|}{Imp.} & \multicolumn{2}{c|}{-2.44\%} & \multicolumn{2}{c|}{-2.70\%} & \multicolumn{2}{c|}{-2.05\%} & \multicolumn{2}{c|}{-6.40\%} & \multicolumn{2}{c|}{-3.01\%} & \multicolumn{2}{c|}{-6.97\%} & \multicolumn{2}{c|}{-6.18\%} & \multicolumn{2}{c|}{-1.22\%} \\

\bottomrule
\end{tabular}
}
\label{tab:main_univariate}
\vspace{-5mm}
\end{table}

==> Tables/mul_main_backup.tex <==
\begin{table}[]
\caption{ Multivariate results with different prediction lengths $O \in \{96, 192, 336, 720\}$. We set the input length as $I \in \{48, 96, 336\}$. A lower MSE indicates a better prediction and Imp. means MSE reduction rate.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccccccccccccccccccccc@{}}
\toprule
\multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{SCINet} & \multicolumn{2}{c}{Autoformer}  & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{Reformer}  & \multicolumn{2}{c}{LSTNet} & \multicolumn{2}{c}{LSTMa} & \multicolumn{2}{c}{TCN} \\ 
% \cmidrule{3-18}
% \cmidrule{3-4}

\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
\cmidrule(lr){15-16}
\cmidrule(lr){17-18}

\multicolumn{2}{c}{MSE}                                             & base           & our           & base         & our         & base           & our          & base          & our          & base          & our          & base            & our           & base         & our         & base         & our       \\ \midrule

% ETTh1
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ETTh1}}} & \multicolumn{1}{l|}{48}  &0.535 & 0.444 & 0.673 & 0.535 & 0.416 & \textbf{0.384} & 0.687 & 0.573 & 0.739 & 0.641 & 0.627 & 0.559 & 0.694 & 0.581 & 0.566 & 0.486\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 0.645 & 0.534 & 0.828 & 0.567 & \textbf{0.442} & 0.444 & 0.908 & 0.856 & 0.803 & 0.731 & 0.760 & 0.682 & 0.829 & 0.661 & 0.763 & 0.679 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.864 & 0.742 & 0.676 & 0.643 & 0.504 & \textbf{0.491} & 1.372 & 1.113 & 0.886 & 0.768 & 0.928 & 0.790 & 1.052 & 0.862 & 0.941 & 0.932  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.933 & 0.889 & 0.791 & 0.699 & 0.569 & \textbf{0.511} & 1.343 & 1.151 & 0.985 & 0.848 & 1.012 & 0.959 & 1.168 & 0.967 & 1.109 & 1.112   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 0.984 & 0.978 & 0.815 & 0.763 & 0.535 & \textbf{0.521} & 1.393 & 1.391 & 1.199 & 1.048 & 1.115 & 1.097 & 1.461 & 1.393 & 1.160 & 1.148  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c}{-10.75\%} & \multicolumn{2}{c}{-15.02\%} & \multicolumn{2}{c}{-4.57\%} & \multicolumn{2}{c}{-11.13\%} & \multicolumn{2}{c}{-12.44\%} & \multicolumn{2}{c}{-8.62\%} & \multicolumn{2}{c}{-15.28\%} & \multicolumn{2}{c}{-5.33\%}  \\ \midrule


% ETTh2
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ETTh2}}} & \multicolumn{1}{l|}{48}  &0.776 & 0.619 & 1.046 & 0.790 & 0.298 & \textbf{0.281} & 0.956 & 0.644 & 0.852 & 0.678 & 0.893 & 0.679 & 0.882 & 0.575 & 0.904 & 0.639 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 1.609 & 1.173 & 1.949 & 1.212 & 0.386 & \textbf{0.351} & 3.400 & 2.462 & 1.849 & 1.312 & 1.443 & 1.117 & 1.669 & 0.991 & 1.740 & 1.529 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 5.014 & 3.976 & 3.821 & 1.769 & 0.439 & \textbf{0.413} & 5.796 & 4.723 & 3.130 & 2.204 & 3.312 & 2.887 & 3.906 & 2.513 & 2.432 & 2.406  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 4.356 & 3.281 & 3.002 & 1.744 & 0.494 & \textbf{0.424} & 3.901 & 3.788 & 2.934 & 2.237 & 3.973 & 3.054 & 2.976 & 2.180 & 2.965 & 2.904  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 4.201 & 3.477 & 4.756 & 1.800 & 0.450 & \textbf{0.421} & 4.018 & 3.961 & 2.631 & 2.628 & 3.725 & 2.990 & 3.298 & 2.680 & 3.151 & 3.142  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c}{-21.98\%} & \multicolumn{2}{c}{-44.02\%} & \multicolumn{2}{c}{-8.26\%} & \multicolumn{2}{c}{-16.62\%} & \multicolumn{2}{c}{-20.58\%} & \multicolumn{2}{c}{-20.44\%} & \multicolumn{2}{c}{-31.32\%} & \multicolumn{2}{c}{-8.99\%}  \\ \midrule

%ETTm1
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ETTm1}}} & \multicolumn{1}{l|}{48}  & 0.563 & 0.556 & 0.610 & 0.605 & 0.549 & \textbf{0.492} & 0.633 & 0.598 & 0.770 & 0.728 & 0.641 & 0.614 & 0.674 & 0.648 & 0.677 & 0.648  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 0.536 & 0.471 & 0.504 & 0.488 & 0.524 & \textbf{0.455} & 0.640 & 0.543 & 0.777 & 0.641 & 0.548 & 0.536 & 0.705 & 0.592 & 0.676 & 0.594 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.563 & 0.506 & 0.490 & \textbf{0.412} & 0.534 & 0.500 & 1.224 & 0.751 & 0.840 & 0.689 & 0.632 & 0.577 & 0.871 & 0.648 & 0.938 & 0.913   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.697 & 0.573 & 0.746 & \textbf{0.465} & 0.561 & 0.514 & 1.390 & 1.008 & 0.987 & 0.895 & 0.798 & 0.686 & 1.125 & 0.681 & 1.148 & 1.126   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 0.904 & 0.682 & 0.747 & 0.576 & 0.560 & \textbf{0.528} & 1.333 & 1.078 & 1.122 & 1.003 & 0.925 & 0.817 & 0.978 & 0.828 & 1.277 & 1.238  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c}{-13.17\%} & \multicolumn{2}{c}{-16.03\%} & \multicolumn{2}{c}{-8.79\%} & \multicolumn{2}{c}{-21.19\%} & \multicolumn{2}{c}{-12.21\%} & \multicolumn{2}{c}{-8.20\%} & \multicolumn{2}{c}{-20.10\%} & \multicolumn{2}{c}{-4.82\%}  \\ \midrule

%ETTm2
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ETTm2}}} & \multicolumn{1}{l|}{48}  & 0.281 & 0.220 & 0.283 & 0.225 & 0.171 & \textbf{0.169} & 0.295 & 0.214 & 0.464 & 0.329 & 0.292 & 0.283 & 0.274 & 0.249 & 0.362 & 0.254 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  &0.371 & 0.248 & 0.392 & 0.257 & 0.293 & \textbf{0.221} & 0.445 & 0.286 & 0.743 & 0.449 & 0.443 & 0.343 & 0.381 & 0.280 & 0.554 & 0.384 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.566 & 0.551 & 0.743 & 0.486 & 0.309 & \textbf{0.284} & 2.283 & 1.453 & 1.208 & 0.836 & 0.950 & 0.830 & 1.178 & 0.601 & 1.868 & 1.956  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} &1.601 & 1.330 & 1.881 & 1.511 & 0.508 & \textbf{0.405} & 2.479 & 1.764 & 2.239 & 1.425 & 1.610 & 1.019 & 1.479 & 0.745 & 2.769 & 2.773  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 5.476 & 5.037 & 4.094 & 3.751 & 0.502 & \textbf{0.426} & 6.580 & 5.777 & 3.068 & 2.827 & 6.130 & 4.449 & 3.083 & 2.381 & 3.204 & 3.187  \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c}{-16.44\%} & \multicolumn{2}{c}{-23.54\%} & \multicolumn{2}{c}{-13.92\%} & \multicolumn{2}{c}{-28.12\%} & \multicolumn{2}{c}{-28.71\%} & \multicolumn{2}{c}{-20.54\%} & \multicolumn{2}{c}{-31.34\%} & \multicolumn{2}{c}{-11.25\%}  \\  \midrule

%Pump
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Pump}}} & \multicolumn{1}{l|}{48}  & 0.724 & 0.715 & 0.779 & 0.703 & 0.577 & \textbf{0.544} & 0.865 & 0.793 & 0.808 & 0.728 & 0.823 & 0.734 & 0.754 & 0.716 & 0.865 & 0.831 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 0.848 & 0.796 & 0.892 & 0.813 & 0.558 & \textbf{0.538} & 0.831 & 0.870 & 0.826 & 0.760 & 1.016 & 1.007 & 0.813 & 0.766 & 1.037 & 0.970  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.851 & 0.843 & 0.782 & 0.821 & 0.597 & \textbf{0.581} & 1.705 & 1.527 & 1.094 & 0.856 & 1.327 & 1.202 & 0.909 & 0.816 & 1.109 & 1.077  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.922 & 0.951 & 1.026 & 0.986 & 0.661 & \textbf{0.621} & 1.676 & 1.492 & 0.966 & 0.918 & 1.654 & 1.292 & 0.934 & 0.859 & 1.521 & 1.208  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} &1.370 & 1.283 & 0.978 & 0.957 & 0.707 & \textbf{0.619} & 1.704 & 1.699 & 1.328 & 1.218 & 1.608 & 1.642 & 1.464 & 1.244 & 2.075 & 1.546   \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c}{-2.34\%} & \multicolumn{2}{c}{-3.96\%} & \multicolumn{2}{c}{-6.08\%} & \multicolumn{2}{c}{-5.07\%} & \multicolumn{2}{c}{-10.57\%} & \multicolumn{2}{c}{-8.16\%} & \multicolumn{2}{c}{-8.83\%} & \multicolumn{2}{c}{-11.87\%}  \\  \midrule

%AirQuality
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{AirQuality}}} & \multicolumn{1}{l|}{48}  & 0.878 & 0.858 & 1.024 & 0.949 & 0.860 & 0.852 & 0.909 & 0.868 & 1.115 & 0.991 & 1.023 & 0.974 & 0.927 & 0.854 & 0.883 & \textbf{0.836} \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 1.108 & 1.112 & 1.159 & 1.139 & 0.992 & \textbf{0.986} & 1.353 & 1.193 & 1.210 & 1.196 & 1.146 & 1.141 & 1.145 & 1.081 & 1.026 & 0.992   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 1.193 & 1.115 & 1.082 & 1.010 & \textbf{0.911} & 0.922 & 1.796 & 1.595 & 1.473 & 1.345 & 1.231 & 1.156 & 1.644 & 1.376 & 1.246 & 1.163  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} &1.224 & 1.214 & 1.168 & 1.061 & 0.962 & \textbf{0.933} & 1.758 & 1.706 & 1.473 & 1.396 & 1.399 & 1.388 & 1.352 & 1.206 & 1.301 & 1.284  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 2.196 & 1.982 & 1.373 & 1.344 & 1.129 & \textbf{1.079} & 2.914 & 2.985 & 1.723 & 1.671 & 1.826 & 1.921 & 2.475 & 2.333 & 1.442 & 1.426    \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.} & \multicolumn{2}{c}{-3.82\%} & \multicolumn{2}{c}{-5.40\%} & \multicolumn{2}{c}{-1.56\%} & \multicolumn{2}{c}{-5.61\%} & \multicolumn{2}{c}{-5.82\%} & \multicolumn{2}{c}{-1.37\%} & \multicolumn{2}{c}{-9.28\%} & \multicolumn{2}{c}{-3.54\%}  \\  \midrule

\bottomrule
\end{tabular}
}
\label{tab:main_multivariate}
\end{table}

==> Tables/mul_new_main.tex <==
\begin{table}[]
\caption{ Multivariate results with different prediction lengths $O \in \{48, 96, 192, 336, 720\}$. We set the input length as $I \in \{48, 96, 336\}$. A lower MSE indicates a better prediction and the best results in each row are bolded. Imp. means averaged MSE reduction rate for a given model and dataset. Total denotes the averaged MSE reduction rate of a given dataset across all baselines models. The full results, which include invisible length setting, confidence interval, and other datasets, are available in Appendix~\ref{app:fullbench}}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccc|cc|cc|cc|cc|cc|cc|cc||c@{}}
\toprule
\multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{SCINet}  & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{Reformer}  & \multicolumn{2}{c}{LSTNet} & \multicolumn{2}{c}{LSTMa} & \multicolumn{2}{c||}{TCN} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Total}}} \\  

\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
\cmidrule(lr){15-16}
\cmidrule(lr){17-18}

\multicolumn{2}{c}{MSE}                                             & base           & ReLD           & base         & ReLD         & base           & ReLD          & base          & ReLD          & base          & ReLD          & base            & ReLD           & base         & ReLD         & base         & ReLD       \\ \midrule

% ETTh1
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ETTh1}}} & \multicolumn{1}{l|}{96}  & 0.645 & 0.534 & \textbf{0.442} & 0.444 & 0.828 & 0.567 & 0.908 & 0.856 & 0.803 & 0.731 & 0.760 & 0.682 & 0.829 & 0.661 & 0.763 & 0.679 & \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-9.35\%}}}\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.864 & 0.742 & 0.504 & \textbf{0.491} & 0.676 & 0.643 & 1.372 & 1.113 & 0.886 & 0.768 & 0.928 & 0.790 & 1.052 & 0.862 & 0.941 & 0.932 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.933 & 0.889 & 0.569 & \textbf{0.511} & 0.791 & 0.699 & 1.343 & 1.151 & 0.985 & 0.848 & 1.012 & 0.959 & 1.168 & 0.967 & 1.109 & 1.112 
  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 0.984 & 0.978 & 0.535 & \textbf{0.521} & 0.815 & 0.763 & 1.393 & 1.391 & 1.199 & 1.048 & 1.115 & 1.097 & 1.461 & 1.393 & 1.160 & 1.148  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-9.17\%} & \multicolumn{2}{c|}{-3.81\%} & \multicolumn{2}{c|}{-13.63\%} & \multicolumn{2}{c|}{-9.78\%} & \multicolumn{2}{c|}{-12.22\%} & \multicolumn{2}{c|}{-8.05\%} & \multicolumn{2}{c|}{-15.03\%} & \multicolumn{2}{c||}{-3.16\%} \\ \midrule


% ETTh2
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ETTh2}}} & \multicolumn{1}{l|}{96}  &1.609 & 1.173 & 0.386 & \textbf{0.351} & 1.949 & 1.212 & 3.400 & 2.462 & 1.849 & 1.312 & 1.443 & 1.117 & 1.669 & 0.991 & 1.740 & 1.529 & \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-20.92\%}}}\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 5.014 & 3.976 & 0.439 & \textbf{0.413} & 3.821 & 1.769 & 5.796 & 4.723 & 3.130 & 2.204 & 3.312 & 2.887 & 3.906 & 2.513 & 2.432 & 2.406  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 4.356 & 3.281 & 0.494 & \textbf{0.424} & 3.002 & 1.744 & 3.901 & 3.788 & 2.934 & 2.237 & 3.973 & 3.054 & 2.976 & 2.180 & 2.965 & 2.904  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 4.201 & 3.477 & 0.450 & \textbf{0.421} & 4.756 & 1.800 & 4.018 & 3.961 & 2.631 & 2.628 & 3.725 & 2.990 & 3.298 & 2.680 & 3.151 & 3.142  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.} & \multicolumn{2}{c|}{-22.42\%} & \multicolumn{2}{c|}{-8.91\%} & \multicolumn{2}{c|}{-48.89\%} & \multicolumn{2}{c|}{-12.61\%} & \multicolumn{2}{c|}{-20.62\%} & \multicolumn{2}{c|}{-19.57\%} & \multicolumn{2}{c|}{-30.46\%} & \multicolumn{2}{c||}{-3.89\%}  \\ \midrule


%ETTm2
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ETTm2}}} &  \multicolumn{1}{l|}{96}  &0.371 & 0.248 & 0.293 & \textbf{0.221} & 0.392 & 0.257 & 0.445 & 0.286 & 0.743 & 0.449 & 0.443 & 0.343 & 0.381 & 0.280 & 0.554 & 0.384 & \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-22.73\%}}}
 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.566 & 0.551 & 0.309 & \textbf{0.284} & 0.743 & 0.486 & 2.283 & 1.453 & 1.208 & 0.836 & 0.950 & 0.830 & 1.178 & 0.601 & 1.868 & 1.956 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} &1.601 & 1.330 & 0.508 & \textbf{0.405} & 1.881 & 1.511 & 2.479 & 1.764 & 2.239 & 1.425 & 1.610 & 1.019 & 1.479 & 0.745 & 2.769 & 2.773 
  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 5.476 & 5.037 & 0.502 & \textbf{0.426} & 4.094 & 3.751 & 6.580 & 5.777 & 3.068 & 2.827 & 6.130 & 4.449 & 3.083 & 2.381 & 3.204 & 3.187 \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-15.15\%} & \multicolumn{2}{c|}{-17.12\%} & \multicolumn{2}{c|}{-24.29\%} & \multicolumn{2}{c|}{-28.29\%} & \multicolumn{2}{c|}{-28.65\%} & \multicolumn{2}{c|}{-24.85\%} & \multicolumn{2}{c|}{-36.96\%} & \multicolumn{2}{c||}{-6.57\%}  \\  \midrule

%Pump
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Pump}}} & \multicolumn{1}{l|}{96}  & 0.848 & 0.796 & 0.558 & \textbf{0.538} & 0.892 & 0.813 & 0.831 & 0.870 & 0.826 & 0.760 & 1.016 & 1.007 & 0.813 & 0.766 & 1.037 & 0.970  & \multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-7.17\%}}}\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.851 & 0.843 & 0.597 & \textbf{0.581} & 0.782 & 0.821 & 1.705 & 1.527 & 1.094 & 0.856 & 1.327 & 1.202 & 0.909 & 0.816 & 1.109 & 1.077 
 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.922 & 0.951 & 0.661 & \textbf{0.621} & 1.026 & 0.986 & 1.676 & 1.492 & 0.966 & 0.918 & 1.654 & 1.292 & 0.934 & 0.859 & 1.521 & 1.208  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} &1.370 & 1.283 & 0.707 & \textbf{0.619} & 0.978 & 0.957 & 1.704 & 1.699 & 1.328 & 1.218 & 1.608 & 1.642 & 1.464 & 1.244 & 2.075 & 1.546   \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-2.61\%} & \multicolumn{2}{c|}{-6.17\%} & \multicolumn{2}{c|}{-2.49\%} & \multicolumn{2}{c|}{-4.28\%} & \multicolumn{2}{c|}{-10.73\%} & \multicolumn{2}{c|}{-7.49\%} & \multicolumn{2}{c|}{-9.77\%} & \multicolumn{2}{c||}{-13.85\%} \\  \midrule

%AirQuality
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{AirQuality}}} &  \multicolumn{1}{l|}{96}  & 1.121 & 1.112 & 0.992 & \textbf{0.986} & 1.159 & 1.139 & 1.353 & 1.193 & 1.210 & 1.196 & 1.146 & 1.141 & 1.145 & 1.081 & 1.026 & 0.992 &\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-4.34\%}}}  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 1.193 & 1.115 & \textbf{0.911} & 0.922 & 1.082 & 1.010 & 1.796 & 1.595 & 1.473 & 1.345 & 1.231 & 1.156 & 1.644 & 1.376 & 1.246 & 1.163  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 1.224 & 1.214 & 0.962 & \textbf{0.933} & 1.168 & 1.061 & 1.758 & 1.706 & 1.473 & 1.396 & 1.399 & 1.388 & 1.352 & 1.206 & 1.301 & 1.284 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & 2.196 & 1.982 & 1.129 & \textbf{1.079} & 1.373 & 1.344 & 2.914 & 2.985 & 1.723 & 1.671 & 1.826 & 1.921 & 2.475 & 2.333 & 1.442 & 1.426    \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.} & \multicolumn{2}{c|}{-4.47\%} & \multicolumn{2}{c|}{-1.72\%} & \multicolumn{2}{c|}{-4.92\%} & \multicolumn{2}{c|}{-5.87\%} & \multicolumn{2}{c|}{-4.51\%} & \multicolumn{2}{c|}{-0.52\%} & \multicolumn{2}{c|}{-9.63\%} & \multicolumn{2}{c||}{-3.09\%}  \\  \midrule

%Weather
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Weather}}} & \multicolumn{1}{l|}{48}  & 0.292 & \textbf{0.279} & 0.344 & 0.343 & 0.366 & 0.333 & 0.345 & 0.294 & 0.343 & 0.313 & 0.318 & 0.310 & 0.346 & 0.325 & 0.348 & 0.327 &\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-5.08\%}}}\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  &0.393 & \textbf{0.358} & 0.464 & 0.446 & 0.449 & 0.411 & 0.453 & 0.443 & 0.526 & 0.416 & 0.414 & 0.386 & 0.409 & 0.387 & 0.450 & 0.424   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.421 & \textbf{0.398} & 0.516 & 0.491 & 0.472 & 0.448 & 0.530 & 0.498 & 0.659 & 0.673 & 0.464 & 0.461 & 0.420 & 0.416 & 1.018 & 1.005  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.454 & \textbf{0.440} & 0.612 & 0.566 & 0.459 & 0.453 & 0.592 & 0.568 & 0.841 & 0.782 & 0.490 & 0.473 & 0.473 & 0.452 & 1.147 & 1.209  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-5.55\%} & \multicolumn{2}{c|}{-4.21\%} & \multicolumn{2}{c|}{-6.01\%} & \multicolumn{2}{c|}{-6.79\%} & \multicolumn{2}{c|}{-8.66\%} & \multicolumn{2}{c|}{-3.41\%} & \multicolumn{2}{c|}{-4.17\%} & \multicolumn{2}{c||}{-1.88\%}  \\  \midrule


%Commodity
\multicolumn{1}{l|}{\multirow{5}{*}{\rotatebox[origin=c]{90}{Commodity}}} & \multicolumn{1}{l|}{48} & 0.392 & 0.392 & 0.382 & 0.377 & 0.505 & 0.520 & 0.369 & 0.369 & 0.428 & 0.424 & 0.484 & 0.507 & 0.389 & 0.385 & 0.367 & \textbf{0.362}  &\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{-7.47\%}}}\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 0.458 & 0.455 & 0.429 & \textbf{0.412} & 0.523 & 0.520 & 0.465 & 0.461 & 0.510 & 0.494 & 0.551 & 0.556 & 0.414 & 0.429 & 0.458 & 0.473    \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.660 & 0.620 & 0.676 & \textbf{0.511} & 0.782 & 0.599 & 0.778 & 0.651 & 0.587 & 0.539 & 0.663 & 0.616 & 0.803 & 0.516 & 0.545 & 0.548  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 1.200 & 0.958 & 0.865 & \textbf{0.464} & 1.285 & 1.069 & 2.587 & 2.619 & 0.690 & 0.664 & 1.157 & 1.104 & 2.479 & 1.736 & 0.604 & 0.607 \\  \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-6.78\%} & \multicolumn{2}{c|}{-19.00\%} & \multicolumn{2}{c|}{-9.52\%} & \multicolumn{2}{c|}{-3.97\%} & \multicolumn{2}{c|}{-4.01\%} & \multicolumn{2}{c|}{-1.52\%} & \multicolumn{2}{c|}{-15.74\%} & \multicolumn{2}{c||}{0.76\%} \\ 


\bottomrule
\end{tabular}
}
\label{tab:main_multivariate}
\vspace{-3mm}
\end{table}

==> Tables/uni2uni_others.tex <==
\begin{sidewaystable}[]
\centering
\footnotesize
\resizebox{1.1\textheight}{!}{
\begin{tabular}{@{}cccccccccccccccccccccccccc@{}}
\toprule
\multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{SCINet} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{N-BEATS} & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{LogTrans} & \multicolumn{2}{c}{Reformer} & \multicolumn{2}{c}{Transformer} & \multicolumn{2}{c}{DeepAR} & \multicolumn{2}{c}{LSTNet} & \multicolumn{2}{c}{LSTMa} & \multicolumn{2}{c}{TCN} \\ \midrule
\multicolumn{2}{c}{MSE}                                             & base           & our           & base         & our         & base           & our           & base          & our         & base          & our          & base          & our          & base          & our          & base            & our           & base         & our         & base         & our         & base        & our        & base        & our       \\ \midrule

% ECL
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ECL}}} & \multicolumn{1}{l|}{48}  & \makecell{ 0.2234 \\\scriptsize$\pm$0.0035 } & \makecell{ \textbf{0.2191} \\\scriptsize$\pm$0.0058 } & \makecell{ 0.4808 \\\scriptsize$\pm$0.0142 } & \makecell{ 0.5017 \\\scriptsize$\pm$0.0242 } & \makecell{ 0.4912 \\\scriptsize$\pm$0.0371 } & \makecell{ 0.4471 \\\scriptsize$\pm$0.0424 } & \makecell{ 0.3799 \\\scriptsize$\pm$0.0062 } & \makecell{ 0.3681 \\\scriptsize$\pm$0.0074 } & \makecell{ 0.2308 \\\scriptsize$\pm$0.0037 } & \makecell{ 0.2266 \\\scriptsize$\pm$0.0040 } & \makecell{ 0.2457 \\\scriptsize$\pm$0.0048 } & \makecell{ 0.2446 \\\scriptsize$\pm$0.0095 } & \makecell{ 0.2772 \\\scriptsize$\pm$0.0159 } & \makecell{ 0.2746 \\\scriptsize$\pm$0.0175 } & \makecell{ 0.2478 \\\scriptsize$\pm$0.0160 } & \makecell{ 0.2451 \\\scriptsize$\pm$0.0114 } & \makecell{ 0.9229 \\\scriptsize$\pm$0.0728 } & \makecell{ 0.8924 \\\scriptsize$\pm$0.0445 } & \makecell{ 0.4664 \\\scriptsize$\pm$0.0380 } & \makecell{ 0.4810 \\\scriptsize$\pm$0.0309 } & \makecell{ 0.3307 \\\scriptsize$\pm$0.0049 } & \makecell{ 0.3344 \\\scriptsize$\pm$0.0152 } & \makecell{ 0.4129 \\\scriptsize$\pm$0.0260 } & \makecell{ 0.4121 \\\scriptsize$\pm$0.0230 }    \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & \makecell{ 0.2393 \\\scriptsize$\pm$0.0061 } & \makecell{ \textbf{0.2337} \\\scriptsize$\pm$0.0013 } & \makecell{ 0.4046 \\\scriptsize$\pm$0.0150 } & \makecell{ 0.4111 \\\scriptsize$\pm$0.0146 } & \makecell{ 0.4401 \\\scriptsize$\pm$0.0360 } & \makecell{ 0.4236 \\\scriptsize$\pm$0.0382 } & \makecell{ 0.3027 \\\scriptsize$\pm$0.0088 } & \makecell{ 0.2953 \\\scriptsize$\pm$0.0056 } & \makecell{ 0.2692 \\\scriptsize$\pm$0.0068 } & \makecell{ 0.2720 \\\scriptsize$\pm$0.0092 } & \makecell{ 0.2812 \\\scriptsize$\pm$0.0197 } & \makecell{ 0.2818 \\\scriptsize$\pm$0.0044 } & \makecell{ 0.3098 \\\scriptsize$\pm$0.0192 } & \makecell{ 0.3000 \\\scriptsize$\pm$0.0059 } & \makecell{ 0.3011 \\\scriptsize$\pm$0.0380 } & \makecell{ 0.2829 \\\scriptsize$\pm$0.0239 } & \makecell{ 0.9167 \\\scriptsize$\pm$0.0799 } & \makecell{ 0.7863 \\\scriptsize$\pm$0.0744 } & \makecell{ 0.3894 \\\scriptsize$\pm$0.0363 } & \makecell{ 0.3900 \\\scriptsize$\pm$0.0382 } & \makecell{ 0.3969 \\\scriptsize$\pm$0.0117 } & \makecell{ 0.3899 \\\scriptsize$\pm$0.0066 } & \makecell{ 0.4585 \\\scriptsize$\pm$0.0637 } & \makecell{ 0.4282 \\\scriptsize$\pm$0.0252 }    \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & \makecell{ 0.2550 \\\scriptsize$\pm$0.0080 } & \makecell{ \textbf{0.2528} \\\scriptsize$\pm$0.0048 } & \makecell{ 0.2543 \\\scriptsize$\pm$0.0026 } & \makecell{ 0.2602 \\\scriptsize$\pm$0.0034 } & \makecell{ 0.4857 \\\scriptsize$\pm$0.0249 } & \makecell{ 0.4816 \\\scriptsize$\pm$0.0536 } & \makecell{ 0.3280 \\\scriptsize$\pm$0.0107 } & \makecell{ 0.3109 \\\scriptsize$\pm$0.0083 } & \makecell{ 0.7091 \\\scriptsize$\pm$0.0141 } & \makecell{ 0.7050 \\\scriptsize$\pm$0.0247 } & \makecell{ 0.3302 \\\scriptsize$\pm$0.0514 } & \makecell{ 0.3352 \\\scriptsize$\pm$0.0408 } & \makecell{ 0.3269 \\\scriptsize$\pm$0.0108 } & \makecell{ 0.3169 \\\scriptsize$\pm$0.0073 } & \makecell{ 0.4044 \\\scriptsize$\pm$0.0393 } & \makecell{ 0.3726 \\\scriptsize$\pm$0.0336 } & \makecell{ 1.0177 \\\scriptsize$\pm$0.0967 } & \makecell{ 1.0244 \\\scriptsize$\pm$0.0858 } & \makecell{ 0.2969 \\\scriptsize$\pm$0.0248 } & \makecell{ 0.2781 \\\scriptsize$\pm$0.0150 } & \makecell{ 0.4585 \\\scriptsize$\pm$0.0264 } & \makecell{ 0.4140 \\\scriptsize$\pm$0.0140 } & \makecell{ 0.4431 \\\scriptsize$\pm$0.0483 } & \makecell{ 0.4132 \\\scriptsize$\pm$0.0221 }   \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} &  \makecell{ 0.3058 \\\scriptsize$\pm$0.0063 } & \makecell{ 0.2959 \\\scriptsize$\pm$0.0051 } & \makecell{ \textbf{0.2956} \\\scriptsize$\pm$0.0020 } & \makecell{ 0.3001 \\\scriptsize$\pm$0.0024 } & \makecell{ 0.4626 \\\scriptsize$\pm$0.1167 } & \makecell{ 0.4386 \\\scriptsize$\pm$0.0571 } & \makecell{ 0.4249 \\\scriptsize$\pm$0.0466 } & \makecell{ 0.3855 \\\scriptsize$\pm$0.0497 } & \makecell{ 0.8006 \\\scriptsize$\pm$0.0142 } & \makecell{ 0.7426 \\\scriptsize$\pm$0.0367 } & \makecell{ 0.3985 \\\scriptsize$\pm$0.0530 } & \makecell{ 0.3156 \\\scriptsize$\pm$0.0153 } & \makecell{ 0.3680 \\\scriptsize$\pm$0.0372 } & \makecell{ 0.3208 \\\scriptsize$\pm$0.0037 } & \makecell{ 0.4428 \\\scriptsize$\pm$0.0525 } & \makecell{ 0.4240 \\\scriptsize$\pm$0.0192 } & \makecell{ 1.2020 \\\scriptsize$\pm$0.1348 } & \makecell{ 1.2797 \\\scriptsize$\pm$0.1520 } & \makecell{ 0.3150 \\\scriptsize$\pm$0.0146 } & \makecell{ 0.3218 \\\scriptsize$\pm$0.0209 } & \makecell{ 0.4658 \\\scriptsize$\pm$0.0130 } & \makecell{ 0.4720 \\\scriptsize$\pm$0.0553 } & \makecell{ 0.4584 \\\scriptsize$\pm$0.0675 } & \makecell{ 0.3933 \\\scriptsize$\pm$0.0315 }    \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} & \makecell{ 0.3356 \\\scriptsize$\pm$0.0137 } & \makecell{ \textbf{0.3210} \\\scriptsize$\pm$0.0081 } & \makecell{ 0.3317 \\\scriptsize$\pm$0.0012 } & \makecell{ 0.3347 \\\scriptsize$\pm$0.0023 } & \makecell{ 0.6059 \\\scriptsize$\pm$0.0511 } & \makecell{ 0.6156 \\\scriptsize$\pm$0.0476 } & \makecell{ 0.5442 \\\scriptsize$\pm$0.1355 } & \makecell{ 0.4970 \\\scriptsize$\pm$0.0749 } & \makecell{ 0.8239 \\\scriptsize$\pm$0.0317 } & \makecell{ 0.7807 \\\scriptsize$\pm$0.0130 } & \makecell{ 0.3720 \\\scriptsize$\pm$0.0344 } & \makecell{ 0.3393 \\\scriptsize$\pm$0.0425 } & \makecell{ 0.3869 \\\scriptsize$\pm$0.0257 } & \makecell{ 0.3630 \\\scriptsize$\pm$0.0159 } & \makecell{ 0.4423 \\\scriptsize$\pm$0.0215 } & \makecell{ 0.4132 \\\scriptsize$\pm$0.0414 } & \makecell{ 1.3023 \\\scriptsize$\pm$0.0562 } & \makecell{ 1.3310 \\\scriptsize$\pm$0.0606 } & \makecell{ 0.3652 \\\scriptsize$\pm$0.0352 } & \makecell{ 0.3672 \\\scriptsize$\pm$0.0169 } & \makecell{ 0.5900 \\\scriptsize$\pm$0.1022 } & \makecell{ 0.5473 \\\scriptsize$\pm$0.0604 } & \makecell{ 0.4411 \\\scriptsize$\pm$0.0504 } & \makecell{ 0.4581 \\\scriptsize$\pm$0.0375 }  \\  \cmidrule{2-26}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.} &  \multicolumn{2}{c}{-2.54\%} & \multicolumn{2}{c}{2.14\%} & \multicolumn{2}{c}{-3.43\%} & \multicolumn{2}{c}{-5.74\%} & \multicolumn{2}{c}{-2.77\%} & \multicolumn{2}{c}{-5.66\%} & \multicolumn{2}{c}{-5.23\%} & \multicolumn{2}{c}{-5.16\%} & \multicolumn{2}{c}{-1.64\%} & \multicolumn{2}{c}{-0.07\%} & \multicolumn{2}{c}{-3.25\%} & \multicolumn{2}{c}{-4.78\%} \\ 
\midrule

\bottomrule
\end{tabular}
}
% }
\end{sidewaystable}

==> Tables/uni_main.tex <==
\begin{table}[]
\caption{Univariate results with different prediction lengths. The experimental settings are identical to those of multivariate experiments.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccc|cc|cc|cc|cc|cc|cc|cc||c@{}}
\toprule


% \multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{N-BEATS}  & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{LogSparse}  & \multicolumn{2}{c}{Reformer} & \multicolumn{2}{c}{Transformer} & \multicolumn{2}{c}{DeepAR} \\
% \cmidrule{3-18}
% \multicolumn{2}{c}{MSE}                                             & base           & ReLD           & base         & ReLD         & base           & ReLD          & base          & ReLD          & base          & ReLD          & base            & ReLD           & base         & ReLD         & base         & ReLD       \\ \midrule
\multicolumn{2}{c}{Models}                                             & \multicolumn{2}{c}{Pyraformer} & \multicolumn{2}{c}{Autoformer} & \multicolumn{2}{c}{N-BEATS}  & \multicolumn{2}{c}{Informer} & \multicolumn{2}{c}{LogSparse}  & \multicolumn{2}{c}{Reformer} & \multicolumn{2}{c}{Transformer} & \multicolumn{2}{c||}{DeepAR} & \multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{Total}}} \\

% \cmidrule{3-18}
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
\cmidrule(lr){15-16}
\cmidrule(lr){17-18}

\multicolumn{2}{c}{MSE}                                             & base           & ReLD           & base         & ReLD         & base           & ReLD          & base          & ReLD          & base          & ReLD          & base            & ReLD           & base         & ReLD         & base         & ReLD       \\ \midrule


% ETTm1
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ETTm1}}} & \multicolumn{1}{l|}{48}  & 0.029 & \textbf{0.025} & 0.036 & 0.033 & 0.031 & 0.029 & 0.043 & 0.036 & 0.037 & 0.033 & 0.078 & 0.070 & 0.032 & 0.032 & 0.084 & 0.050 & \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{-15.21\%}}} \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 0.082 & 0.058 & 0.058 & \textbf{0.052} & 0.085 & 0.066 & 0.105 & 0.083 & 0.105 & 0.058 & 0.228 & 0.161 & 0.089 & 0.060 & 0.179 & 0.085 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.129 & 0.122 & 0.088 & 0.072 & 0.077 & \textbf{0.070} & 0.181 & 0.158 & 0.192 & 0.161 & 0.284 & 0.223 & 0.221 & 0.196 & 0.200 & 0.199  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} &0.194 & 0.184 & 0.090 & \textbf{0.085} & 0.134 & 0.125 & 0.263 & 0.227 & 0.367 & 0.304 & 0.339 & 0.304 & 0.274 & 0.247 & 0.382 & 0.432  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} &0.337 & 0.275 & 0.143 & 0.112 & 0.144 & \textbf{0.112} & 0.391 & 0.349 & 0.474 & 0.381 & 0.396 & 0.410 & 0.479 & 0.443 & 0.498 & 0.418  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-13.98\%} & \multicolumn{2}{c|}{-12.69\%} & \multicolumn{2}{c|}{-12.88\%} & \multicolumn{2}{c|}{-15.03\%} & \multicolumn{2}{c|}{-21.83\%} & \multicolumn{2}{c|}{-13.76\%} & \multicolumn{2}{c|}{-12.20\%} & \multicolumn{2}{c||}{-19.35\%}  \\ \midrule


% ECL
\multicolumn{1}{l|}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ECL}}} & \multicolumn{1}{l|}{48}  & 0.223 & \textbf{0.219} & 0.491 & 0.447 & 0.380 & 0.368 & 0.231 & 0.227 & 0.246 & 0.245 & 0.277 & 0.275 & 0.248 & 0.245 & 0.923 & 0.892 & \multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{-4.02\%}}}\\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{96}  & 0.239 & \textbf{0.234} & 0.440 & 0.424 & 0.303 & 0.295 & 0.269 & 0.272 & 0.281 & 0.282 & 0.310 & 0.300 & 0.301 & 0.283 & 0.917 & 0.786 \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{168} & 0.255 & \textbf{0.253} & 0.486 & 0.482 & 0.328 & 0.311 & 0.709 & 0.705 & 0.330 & 0.335 & 0.327 & 0.317 & 0.404 & 0.373 & 1.018 & 1.024  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{336} & 0.306 & \textbf{0.296} & 0.463 & 0.439 & 0.425 & 0.386 & 0.801 & 0.743 & 0.399 & 0.316 & 0.368 & 0.321 & 0.443 & 0.424 & 1.202 & 1.280  \\

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{720} &0.336 & \textbf{0.321} & 0.606 & 0.616 & 0.544 & 0.497 & 0.824 & 0.781 & 0.372 & 0.339 & 0.387 & 0.363 & 0.442 & 0.413 & 1.302 & 1.331  \\ \cmidrule{2-18}

\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{Imp.}& \multicolumn{2}{c|}{-2.54\%} & \multicolumn{2}{c|}{-3.43\%} & \multicolumn{2}{c|}{-5.74\%} & \multicolumn{2}{c|}{-2.77\%} & \multicolumn{2}{c|}{-5.66\%} & \multicolumn{2}{c|}{-5.23\%} & \multicolumn{2}{c|}{-5.16\%} & \multicolumn{2}{c||}{-1.64\%} \\

\bottomrule
\end{tabular}
}
\label{tab:main_univariate}
\vspace{-5mm}
\end{table}
